Cross-Domain Correlation Distillation for Unsupervised Domain Adaptation in Nighttime Semantic Segmentation

The performance of nighttime semantic segmentation is restricted by the poor illumination and a lack of pixel-wise annotation, which severely limit its application in autonomous driving. Existing works, e.g., using the twilight as the intermediate target domain to perform the adaptation from daytime to nighttime, may fail to cope with the inherent difference between datasets caused by the camera equipment and the urban style. Faced with these two types of domain shifts, i.e., the illumination and the inherent difference of the datasets, we propose a novel domain adaptation framework via cross-domain correlation distillation, called CCDistill. The invariance of illumination or inherent difference between two images is fully explored so as to make up for the lack of labels for nighttime images. Specifically, we extract the content and style knowledge contained in features, calculate the degree of inherent or illumination difference between two images. The domain adaptation is achieved using the invariance of the same kind of difference. Extensive experiments on Dark Zurich and ACDC demonstrate that CCDistill achieves the state-of-the-art performance for nighttime semantic segmentation. Notably, our method is a one-stage domain adaptation network which can avoid affecting the inference time. Our implementation is available at https://github.com/ghuan99/CCDistill.

==> bdd.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{bdd.PNG}
\hfill
%\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
The qualitative comparison of our approach and some existing state-of-the-art methods on the BDD100K-night set.
}
\label{fig:bdd}
\end{figure*}

==> rebuttalablations.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{1mm}{ %< auto-adjusts font size to fill line
\setlength{\abovecaptionskip}{0.1pt}
\caption{
% 
Ablation studies of our method on Dark Zurich-test.
% 
} % \caption
\setlength{\belowcaptionskip}{0.1pt}
\label{tab:rebuttalablations}
\scalebox{0.8}{
\begin{tabular}{@{}l|c|c@{}}
\hline
Method & w/o CDC and CDS & w/ only one model $M$  \\
\hline
mIoU &  44.8 & 43.8\\
\hline
\end{tabular}
}
} %< \resizebox
\vspace{-1.0em}
\end{table}

==> rebuttalcomparisons.tex <==
\begin{table}
\centering
\setlength{\abovecaptionskip}{0.1pt}
\caption{
% 
Comparison with SOTA approaches on Dark Zurich-val.
% 
} % \caption
\setlength{\belowcaptionskip}{0.1pt}
\label{tab:rebuttalcomparisons}
\scalebox{0.8}{
\begin{tabular}{@{}c|c|c|c@{}}
\hline
Method & MGCDA & DANNet & Ours  \\
\hline
mIoU &  25.3 & 33.9 & 35.7 \\
\hline
\end{tabular}
}
\vspace{-2.0em}
\end{table}


==> supplement_acdc.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{latex/fig/supplement_acdc.PNG}
\hfill
%\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\setlength{\abovecaptionskip}{1pt}
\caption{
% 
The qualitative comparison between our approach and some existing state-of-the-art methods on the ACDC-night-val set.
}
\setlength{\belowcaptionskip}{1pt}
\label{fig:supplement_acdc}
\end{figure*}

==> supplement_bdd.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{latex/fig/supplement_bdd.PNG}
\hfill
%\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\setlength{\abovecaptionskip}{1pt}
\caption{
% 
The qualitative comparison between our approach and some existing state-of-the-art methods on the BDD100K-night set.
}
\setlength{\belowcaptionskip}{1pt}
\label{fig:supplement_bdd}
\end{figure*}

==> supplement_val.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{latex/fig/supplement_val.PNG}
\hfill
%\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\setlength{\abovecaptionskip}{1pt}
\caption{
% 
The qualitative comparison between our approach and some existing state-of-the-art methods on the Dark Zurich-val set.
}
\setlength{\belowcaptionskip}{1pt}
\label{fig:supplement_val}
\end{figure*}
